My CXL Pool Obviates Your PCIe Switch

Pooling PCIe devices across multiple hosts offers a promising solution to mitigate stranded I/O resources, enhance device utilization, address device failures, and reduce total cost of ownership. The only viable option today are PCIe switches, which decouple PCIe devices from hosts by connecting them through a hardware switch. However, the high cost and limited flexibility of PCIe switches hinder their widespread adoption beyond specialized datacenter use cases. This paper argues that PCIe device pooling can be effectively implemented in software using CXL memory pools. CXL memory pools improve memory utilization and already have positive return on investment. We find that, once CXL pools are in place, they can serve as a building block for pooling any kind of PCIe device. We demonstrate that PCIe devices can directly use CXL memory as I/O buffers without device modifications, which enables routing PCIe traffic through CXL pool memory. This software-based approach is deployable on today's hardware and is more flexible than hardware PCIe switches. In particular, we explore how disaggregating devices such as NICs can transform datacenter infrastructure.

==> acknowledgments.tex <==
\section{Acknowledgments}

We would like to thank the anonymous reviewers for their comments. We thank Frank Hady and Andrew Ruffin for their generous equipment support,
and to Adam Manzanares, Cyril Guyot, Qing Li and Filip Blagojevic for their feedback throughout the project.
This work was in part supported by ARO grant W911NF-21-1-0078, ONR grants N00014-16-1-2263 and N00014-17-1-2788; NSF grants CNS-2104292, CNS-1750558 and CNS-15-64055; an Intel equipment donation; a JP Morgan Faculty Research Award; and a DiDi Faculty Research Award.

==> challenges.tex <==
\section{Research Challenges}

Our initial experiments demonstrate that when issuing successive dependent storage requests, BPF can
provide significant speedups of more than 2.5$\times$. %However,
%there remain significant challenges in using BPF to accelerate storage lookups
%for a practical system such as a key-value store.
%
%\paragraph{Compatibility with existing storage stack.}
%
% Our first set of challenges arises from our desire to remain to compatible with
% Linux and its existing storage stack.
% The first question is where to place the kernel hook that calls the BPF functions, which
% will issue the NVMe requests.
% Our initial results show that to be effective at improving storage latency
% and throughput, I/O resubmissions must happen as early as possible after an
% I/O completes to avoid wasted work, ideally within the kernel NVMe interrupt
% handler itself. 
% Therefore, in the rest of this section, we presume the resubmissions occur in the NVMe driver.
% However, allowing user-defined functions to submit I/Os from
% the NVMe interrupt handler requires us to not to violate various file system guarantees (\eg security, isolation)
% without having the full context of a file system.
% \textbf{Where to place the kernel hook.}
%
%The first question is where to place the kernel hook that calls the BPF functions to
%reissue the NVMe requests.
However, to realize these gains, I/O resubmissions must happen as early as possible,
ideally within the kernel NVMe interrupt
handler itself. %, to be effective at improving storage latency
%and throughput.
%Therefore, in the rest of this section, we assume that resubmissions occur in the NVMe driver.
This creates significant challenges in using BPF to accelerate storage lookups
for a practical system such as a key-value store.
%However, allowing user-defined functions to submit I/Os from
%the NVMe interrupt handler creates the following challenges.
%As we showed earlier, bypassing the file system and bio layer, and issuing the requests directly
%to the NVMe layer, provides a much higher
%potential speedup (4$\times$) compared to issuing the requests from the system call handling layer (1.15$\times$).
%Therefore, in the rest of this section, we presume the resubmissions occur in the NVMe driver.
%However, this creates several significant challenges.

%\missingfigure{Graph of FS vs bio vs NVMe driver}

\paragraph{Interface.} The goal of the kernel resubmission mechanism is to efficiently traverse an
application-defined data structure (\eg an index or a database table).
Therefore, we want to provide a general-purpose Linux-compatible interface for the application to
define data structure layout and to allow the kernel to traverse it using BPF.
Beyond the challenge of designing a general-purpose interface, there are three other challenges.

First, the data structure can be defined using physical disk addresses and offsets, or based on the file system addresses. The former reduces metadata and communication with the file system layer, but may lead to incorrect address translation when the file system restructures files (as well as create security issues, see below). The latter would require synchronization with the file system layer.
Second, the NVMe driver relies on the BIO layer's queues to ensure that it will not overflow the actual hardware queue on the NVMe device.
Normally, one contiguous extent of a file could be split into multiple NVMe requests at the block layer.
But supporting fanout while reissuing within the NVMe interrupt handler is  problematic
because the handler would have to allocate memory for additional NVMe requests
and coordinate with the ordinary submission path within an interrupt context.
Instead, the interrupt handler can only reuse the NVMe request that just completed,
which may limit the types of data structures and traversals we can support
to those without fanout.
Third, applications often partially cache on-disk indices. We need to ensure
that the BPF traversal does not adversely impact these caches.

\paragraph{Security.} In Linux the NVMe layer doesn't have access to file system metadata.
%, and our
%results show that it is cost-prohibitive to submit I/Os from the file system
%layer.
If an I/O completes for a block at offset $o_1$ in a file, a
user-defined function might extract file offset $o_2$ as the next I/O
to issue. However, $o_2$ is meaningless to the NVMe
context, since it cannot tell which physical block this corresponds to
without access to the file's metadata and extents. Blocks could embed
physical block addresses to avoid the need to consult the extents, but without
imposing limits on these addresses, user-defined functions could access any
block on the device. Hence, 
%the extents are necessary to validate
%which blocks the function should be allowed to access.
a key challenge is imbuing the NVMe layer with enough information to
efficiently and safely map file offsets to the file's corresponding physical
block offsets without restricting the file system's ability to remap blocks
as it chooses.
%\textbf{Bandwidth vs Latency.}

\paragraph{Concurrency \& fairness.} Enabling concurrent reads and writes across BPF and the file system within the same file will be difficult.
%A write issued through the file system could conflict with a BPF traversal, even if that traversal is read-only.
A write issued through the file system might only be reflected in the buffer cache,
and would not be visible to the BPF traversal.
This could be addressed by locking, but managing locks from within the NVMe driver could be expensive.
Therefore,
data structures that require fine-grained locking (\eg lock crabbing in B+trees)
require careful design to support BPF traversal.

In a multi-tenant scenario, since the BPF issued requests do not go through the file system or block layer,
there is no clear enforcement of fairness or QoS guarantees.
In any case, the default block layer scheduler in Linux is already the nop scheduler for NVMe devices,
and the NVMe specification enables command arbitration at the hardware queue level if fairness is a requirement~\cite{nvme-spec}.
Another challenge is that the NVMe layer
may reissue an infinite number of I/O requests.
The eBPF verifier prevents loops with unknown bounds~\cite{bpf-verification},
but if we add a hook in the NVMe interrupt handler, we would also need to prevent such loops.

==> conclusions.tex <==
\section{Conclusions}

